ReLeQ: A Reinforcement Learning Approach for Deep Quantization of Neural Networks

Deep Neural Networks (DNNs) typically require massive amount of computation resource in inference tasks for computer vision applications. Quantization can significantly reduce DNN computation and storage by decreasing the bitwidth of network encodings. Recent research affirms that carefully selecting the quantization levels for each layer can preserve the accuracy while pushing the bitwidth below eight bits. However, without arduous manual effort, this deep quantization can lead to significant accuracy loss, leaving it in a position of questionable utility. As such, deep quantization opens a large hyper-parameter space (bitwidth of the layers), the exploration of which is a major challenge. We propose a systematic approach to tackle this problem, by automating the process of discovering the quantization levels through an end-to-end deep reinforcement learning framework (ReLeQ). We adapt policy optimization methods to the problem of quantization, and focus on finding the best design decisions in choosing the state and action spaces, network architecture and training framework, as well as the tuning of various hyperparamters. We show how ReLeQ can balance speed and quality, and provide an asymmetric general solution for quantization of a large variety of deep networks (AlexNet, CIFAR-10, LeNet, MobileNet-V1, ResNet-20, SVHN, and VGG-11) that virtually preserves the accuracy (=< 0.3% loss) while minimizing the computation and storage cost. With these DNNs, ReLeQ enables conventional hardware to achieve 2.2x speedup over 8-bit execution. Similarly, a custom DNN accelerator achieves 2.0x speedup and energy reduction compared to 8-bit runs. These encouraging results mark ReLeQ as the initial step towards automating the deep quantization of neural networks.

==> body/ablation_studies.tex <==
\section{Ablation Studies and Discussion}
% (add something?)
\subsection{Influence of Reward Function}\label{sec:reward}
%
The design of reward function is a crucial component of reinforcement learning as indicated in section \ref{sec:Reward}.
%
There are many possible reward functions one could define for a particular application setting. However, different designs could lead to either different policies or different convergence behavior.
%
In this paper, we incorporate reward engineering by proposing special parametric reward formulation. First, we argue that the proposed formulation helps to achieve better final performance during fixed amount of training episodes (performance here can be interpreted either as better final solution quality or faster convergence time). Second, in this context of multi-objective optimization, where there are a set of optimal solutions (defined by the Pareto frontier), the actual cost-benefit tradeoff (accuracy state vs quantization state) is controlled by having a parametric formulation.
%
To evaluate the effectiveness of the proposed reward formulation, we have compared three different reward formulations: $(i)$ proposed in section \ref{sec:Reward}, $(ii) R=acc_st/quant_st$, $(iii) R=acc_st-quant_st$. Figure \ref{fig:diff_rewards} summarizes the convergence behavior for the three formulations. 
%
The proposed reward formulation consistently shows higher performance in terms of faster convergence time and better solution quality as compared to others.
%

\iffalse 
\subsection{Evaluation of State Embeddings}
State embeddings are an essential component in determining and controlling the convergence behavior of the RL agent. We carried out experiments to evaluate the effectiveness of the used state embeddings. In every iteration, we repeat the same experiment while omitting one state embedding at a time and keeping the rest. Based on our experiments, we observe that the layer's size/dimensions turn out to be the most important embedding for convergence. Standard deviation of the layer's weights comes as the second most important parameter. Figure \ref{fig:wo-weight-stat} shows convergence behavior for LeNet with variance of weights as part of the state embedding (baseline result) and Figure \ref{fig:w-weight-stat} shows the behavior when variance of weights was excluded from the state embedding. The rest of the state embeddings help in speeding up the convergence process.
%
\begin{figure}
\centering
\begin{subfigure}{0.4\textwidth}
  \centering\includegraphics[width=\textwidth]{figs/probs-wo-weight-stats}
  \caption{Excluding weight variance in the state embedding}
    \label{fig:wo-weight-stat}
\end{subfigure}
%
\begin{subfigure}{0.4\textwidth}
  \centering\includegraphics[width=\textwidth]{figs/probs-w-weight-stats}
  \caption{Including weight variance in the state embedding}
    \label{fig:w-weight-stat}
\end{subfigure}
\caption{Comparison of ReLeQ convergence performance for LeNet (convolution layer 1) on MNIST dataset (a) when weight variances are excluded from the state embedding and (b) when weight variances are included in the state embedding	.}
\label{fig:weight_stats}
\end{figure}
%
\fi

\subsection{Tuning PPO clipping parameter}\label{sec:clipping_param_tuning}
One of the unique features about PPO algorithm is its novel objective function with clipped probability ratios, which forms a pessimistic estimate
(i.e., lower bound) of the performance of the policy. Such modification restricts the range that the new policy can vary from the old one, hence improves the stability of the learning process.  With Clipped Surrogate Objective function, we have two probability ratios, one non clipped and one clipped in a range between $\lbrack1-\epsilon$, $1+\epsilon\rbrack$, where $\epsilon$ is a hyper parameter that helps to define this clip range. Table \ref{table:clipping_table} provides a summary of tuning epsilon (commonly in the range of 0.1, 0.2, 0.3). Based on our performed experiments, $\epsilon=0.1$ often reports the highest average reward across different benchmarks.


==> body/background.tex <==
%\section{Background}
%\subsection{Deep Reinforcement Learning}
%Recent advancements in combining deep learning techniques with reinforcement learning have led to phenomenal feats like Deepmind's AlphaZero which learns to play with zero human intervention and OpenAI Five, a team of five networks which has been defeating human teams in Dota 2. While deep learning enables us to understand unstructured environments, reinforcement learning provides a formalism for behavior and both of these combined allow us to solve much more complex problems in an unsupervised environment. Neural Fitted Q Learning (NFQ) was one of the first efforts in combining these two fields but the major breakthrough in Deep Reinforcement Learning was with introduction of Deep Q-Networks(DQNs), which could master a diverse set of Atari games and surpass human performance. And from that point on, improvements in DQNs and new methods such as Policy Gradients have accelerated the progress in Deep Reinforcement Learning.
%
%\subsection{Proximal Policy Optimization}\label{sec:PPO}
%
%Policy Gradient Methods have played central part in the recent breakthroughs in Deep Reinforcement Learning and these algorithms aim to address some of the disadvantages of using value based methods (DQNs) like big oscillations while training, inefficiency in handling large action spaces and the inability to learn stochastic policies. We use Proximal Policy Optimization(PPO), which is the state-of-the art algorithm based on Policy Gradient Method to train our RL agent. While most standard policy gradient algorithms perform only one gradient update per batch, PPO enables multiple epochs of updates per batch. PPO also avoids too large policy updates by clipping the probability ratios between old and new policies to the range of 0.8 to 1.2.
%
%\subsection{Related Work}


\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.9\textwidth]{figs/block_diagram_2.pdf}
    \caption{Overview of ReLeQ framework.}		  
    \label{fig:block_diagram}
%    \vspace{0.2cm}
\end{figure*}


==> body/evaluation.tex <==
%
\section{Experimental Results}
\vspace{-1ex}
%
%\paragraph{Benchmarks.} To demonstrate the effectiveness of ReLeQ, we conducted experiments on a variety of neural networks (AlexNet, CIFAR10, LeNet, MobileNet, ResNet-20, SVHN, and VGG11) on different datasets (CIFAR10, ImageNet, MNIST and SVHN). The goal of each experiment is to find a quantization policy for each layer which optimally strikes a balance between minimizing the total compute cost and maintaining the accuracy within a recoverable level. 
%

\begin{figure}
\centering 	
 	\includegraphics[width=0.45\textwidth]{figs/enum_4nets.pdf}
	\caption{Quantization space and its Pareto frontier for  
	(a) CIFAR-10, (b) LeNet, (c) SVHN, and (d) VGG-11.}
	\label{fig:enum}
	\vspace{-0.5cm}
 \end{figure}

\paragraph{Quantization levels with \releq.}\label{sec:quant_policy}
%
Table~\ref{table:networks} provides a summary of the evaluated networks, datasets and shows the results with respect to layer-wise quantization levels (bitwidths) achieved by \releq. 
%
%In the context of automatic deep quantization of neural networks, quantization policy is defined as the course of layer-wise bitwidth selection proposed by the agent for a particular neural network. Such a policy comprises two aspects, the quantization pattern of layer-wise bitwidths and the implications on the optimization objective. 
%
Regarding the layer-wise quantization bitwidths, at the onset of the agent's exploration, all layers are initialized to 8-bits.
%
As the agent learns the optimal policy, each layer converges with a high probability to a particular quantization bitwidth. 
%
As shown in the \bench{``Bitwidths''} column of  Table~\ref{table:main_results}, \releq quantization policies show a spectrum of varying bitwidth assignments to the layers.
%
The bitwidth for MobileNet varies from 4 bits to 8 bits with an irregular pattern, which averages to 6.43.
%
ResNet-20 achieves mostly 2 and 3 bits, again with an irregular interleaving that averages to 2.81.
%
In many cases, there is significant heterogeneity and irregularity in the bitwidths and a uniform assignment of the bits is not always the desired choice to preserve accuracy.
%
%
These results demonstrate that ReLeQ automatically distinguishes different layers and their varying importance with respect to accuracy while choosing their respective bitwidths.
%
As shown in the \bench{``Accuracy Loss''} column of  Table~\ref{table:networks}, the deeply quantized networks with \releq have less than 0.30\% loss in classification accuracy. 
%
%Moreover, these results defeat other empirical quantization policies which either assign same bitwidth to all layers~\cite{Choi2018PACTPC}, or propose heterogenous allocation yet suboptimal~\cite{Ye2018AUF}.
%
To assess the quality of these bitwidth assignments, we conduct a Pareto analysis on the DNNs for which we could populate the search space.
%

\begin{figure*}
\centering
    \includegraphics[width=0.8\textwidth]{figs/conv_graphs_2.pdf}
    \caption{The evolution of reward and its basic elements, (a), (b) State of Relative Accuracy and (c), (d) State of Quantization) as the agent learns through the episodes.
    The last plot (e) shows an alternative view by depicting the evolution of reward for MobileNet.
    The trends are similar for the other networks.
    }
    \label{fig:convergence}
\vspace{-3ex}
\end{figure*}


\niparagraph{Validation: Pareto analysis.}\label{sec:Validation}
%
Figure \ref{fig:enum} depicts the solutions space for four benchmarks (CIFAR10, LeNet, SVHN, and VGG11).
%
Each point on these charts is a unique combination of bitwidths that are assigned to the layers of the network.
%
The boundary of the solutions denotes the Pareto frontier and is highlighted by a dashed line.
%
The solution found by \releq is marked out using an arrow and lays on the desired section of the Pareto frontier where the accuracy loss can be recovered through fine-tuning.
%
It is worth noting that as a result of the moderate size of the four networks presented in this subsection, it was possible to enumerate the design space, obtain Pareto frontier and assess ReLeQ quantization policy for each of the four networks. 
%
However, it is infeasible to do so for state-of-the-art deep networks (e.g., MobileNet and AlexNet) which further stresses the importance of automation and efficacy of \releq.

\niparagraph{Learning and convergence analysis.}\label{sec:Convergence}
%
We further study the desired behavior of \releq in the context of convergence.
%
An appropriate evidence for the correctness of a formulated reinforcement learning problem is the ability of the agent to consistently yield improved solutions.
%
The expectation is that the agent learns the correct underlying policy over the episodes and gradually transitions from the exploration to the exploitation phase. 
%
Figures~\ref{fig:convergence}(a) and (b) first show the \bench{State of Relative Accuracy} for CIFAR10 and SVHN, respectively. 
%
We overlay the moving average of \bench{State of Relative Accuracy} as episodes evolve, which is denoted by a black line in Figures~\ref{fig:convergence}(a) and (b).
%
Similarly, Figures~\ref{fig:convergence}(c) and (d) depict the evolution of \bench{State of Quantization}. 
%
As another indicative parameter of learning, Figure~\ref{fig:convergence} plots the evolution of the reward, which combines the two \bench{States of Accuracy} and \bench{Quantization} (Section~\ref{sec:reward}).
%
As all the graphs show, the agent consistently yields solutions that increasingly preserve the accuracy (maximize rewards), while seeking to minimize the number of bits assigned to each layer (minimizing the state of quantization) and eventually converges to a rather stable solution. 
%
The trends are similar for the other networks.

%
%For the SVHN experiment, we run multi-digit recognition (five digits with ten classes for each digit) using a ten layer network. During the experiment, we set the first and last layers as full precision (excluding them from the search space).


 \begin{figure}
	\centering\includegraphics[width=0.45\textwidth]{figs/tvm.pdf}
	\caption{Speedup with \releq for conventional hardware using TVM over the baseline run using 8 bits.}
	\label{fig:tvm}
	\vspace{-1ex}
\end{figure}
	
 \begin{figure}
	\centering\includegraphics[width=0.45\textwidth]{figs/stripes.pdf}
	\caption{Energy reduction and speedup with \releq for Stripes over the baseline execution when the accelerator is running 8-bit DNNs.}
	\label{fig:stripes}
	\vspace{-0.5cm}
\end{figure}

\begin{table*}
	\centering
	\caption{Speedup and energy reduction with \releq over the benefits with ADMM~\cite{Ye2018AUF} over the two networks that ADMM reports. The improvements with \releq is reported with both TVM and Stripes.}
	\includegraphics[width=0.65\linewidth]{figs/res_comparison.pdf}
	\label{table:res_comp}
	\vspace{-0.3cm}
\end{table*}

\begin{figure*}
  	  \centering\includegraphics[width=0.8\textwidth]{figs/diff_rewards.pdf}
	  \caption{Three different reward functions and their impact on the state of relative accuracy over the training episodes for three different networks. (a) CIFAR10, (b) LeNet, and (c) SVHN.}
	  \label{fig:diff_rewards}
	  \vspace{-3ex}
 \end{figure*}


\niparagraph{Execution time and energy benefits with \releq.} 
%
Figure~\ref{fig:tvm} shows the speedup for each benchmark network conventional hardware using TVM compiler. 
%
The baseline is the 8-bit runtime for inference. 
%
\releq's solution offers, on average, $2.2\times$ speedup over the baseline as the result of merely quantizing the weights that reduces the amount of computation and data transfer during inference. 
%
Figure~\ref{fig:stripes} shows the speedup and energy reduction benefits of \releq's solution on Stripes custom accelerator. 
%
The baseline here is the time and energy consumption of 8-bit inference execution on the same accelerator.
%

\releq's solutions yield, on average, $2.0\times$ speedup and an additional $2.0\times$ energy reduction. 
%
MobileNet achieves $1.2\times$ speedup which is coupled with a similar degree of energy reduction.
%
On the other end of the spectrum ResNet-20 and LeNet achieve $3.0\times$ and $4.0\times$ the benefits, respectively.
%
As shown in Table~\ref{table:networks}, MobileNet needs to be quantized to higher bitwidths to maintain accuracy, compared with other networks and that is why the benefits are smaller. 

\niparagraph{Speedup and energy reduction over ADMM.} 
%
As mentioned in Section~\ref{sec:exp}, we compare \releq's solution in terms of speedup and energy reduction against ADMM~\cite{Ye2018AUF}, another procedure for finding quantization bitwidths. 
%
As shown in Table~\ref{table:res_comp}, \releq's solution provides $1.25\times$ energy reduction and $1.22\times$ average speedup over ADMM with Stripes for AlexNet and the benefits are higher for LeNet.
%
The benefits are similar for the conventional hardware using TVM as shown in Table~\ref{table:res_comp}.
%
ADMM does not report other networks.




\niparagraph{Sensitivity analysis: influence of reward function.}\label{sec:rewardsens}
%
%
The design of reward function is a crucial component of reinforcement learning as indicated in Section~\ref{sec:reward}.
%
There are many possible reward functions one could define for a particular application setting. However, different designs could lead to either different policies or different convergence behavior.
%
In this paper, we incorporate reward engineering by proposing a special parametric reward formulation.
%
To evaluate the effectiveness of the proposed reward formulation, we have compared three different reward formulations in Figure \ref{fig:diff_rewards}: (a) proposed in Section~\ref{sec:reward}, (b) $ R=State_{Accuracy}/State_{Quantization}$, (c) $ R=State_{Accuracy}-State_{Quantization}$.
%
As the blue line in all the charts shows, the proposed reward formulation consistently achieves higher \bench{State of Relative Accuracy} during the training episodes.
% 
That is, our proposed reward formulation enables \releq finds better solutions in shorter time.

\niparagraph{Tuning: PPO objective clipping parameter.}\label{sec:clipping_param_tuning}
%
One of the unique features about PPO algorithm is its novel objective function with clipped probability ratios, which forms a lower-bound estimate of the change in policy. 
%
Such modification controls the variance of the new policy from the old one, hence improves the stability of the learning process.
%
PPO uses a Clipped Surrogate Objective function, which uses the minimum of two probability ratios, one non-clipped and one clipped in a range between $\lbrack1-\epsilon$, $1+\epsilon\rbrack$, where $\epsilon$ is a hyper-parameter that helps to define this clipping range. 
%
Table \ref{table:clipping_table} provides a summary of tuning epsilon (commonly in the range of 0.1, 0.2, 0.3). Based on our performed experiments, $\epsilon=0.1$ often reports the highest average reward across different benchmarks.

\begin{table}
	\centering
	\caption{Sensitivity of reward to different clipping parameters.}
	\includegraphics[width=0.9\linewidth]{figs/clipping_table.pdf}
	\label{table:clipping_table}
	\vspace{-0.5cm}
\end{table}



==> body/experimental_setup.tex <==
\section{Experimental Setup}
\vspace{-3ex}
\label{sec:exp}
 \begin{table}[!h]
	\centering
	\caption{Benchmark DNNs and their deep quantization with \releq.}
	\includegraphics[width=0.95\linewidth]{figs/results_summary_table.pdf}
	\label{table:networks}
	\vspace{-0.5cm}
\end{table}
%
\vspace{-0.2cm}
\paragraph{Benchmarks.}
%
To assess the effectiveness of \releq across a variety of DNNs, we use the following seven diverse networks that have been used in different real-world vision tasks: AlexNet, CIFAR-10 (simplenet), LeNet, MobileNet (Version 1), ResNet-20, SVHN and VGG-11.
%
Of these seven networks, AlexNet and MobileNet were evaluated on the ImageNet (ILSVRC'12) dataset, ResNet-20, VGG-11 and CIFAR-10 on CIFAR-10, SVHN on SVHN  and LeNet on the MNIST dataset.  

\vspace{-0.2cm}
\paragraph{Quantization technique.} We use the technique proposed in WRPN \cite{Mishra2017WRPNWR} where weights are first scaled and clipped to the $(-1.0, 1.0)$ range and quantized as per the following equation. 
%
The term $k$ is the bitwidth used for quantization out of which $k-1$ bits are used for quantization and one bit is used for sign.
%
\begin{small}
\vspace{-2ex}
	$$ x_{q} = \frac{round((2^{k-1} - 1)x_{f})}{2^{k-1} - 1}$$
	\vspace{-3ex}
\end{small}

\vspace{-0.5cm}
\paragraph{Deep quantization with conventional hardware.} \releq's solution can be deployed on conventional hardware, such as general purpose CPUs to provide benefits and improvements. 
%
To manifest this, we have evaluated \releq using TVM~\cite{TVM} on an Intel Core i7-4790 CPU.
%
We use TVM since its compiler supports deeply quantized operations with bit-serial vector operations on conventional hardware. 
%
We compare our solution in terms of the inference execution time (since the TVM framework does not offer energy measurements) against 8-bit quantized network. 
%
The results can be seen in Figure~\ref{fig:tvm} and will be further elaborated in the next section.

\vspace{-0.5cm}
\paragraph{Deep quantization with custom hardware accelerators.} To further demonstrate the energy and performance benefits of the solution found by \releq, we evaluate it on Stripes~\cite{stripes}, a custom accelerator designed for DNNs, which exploits bit-serial computation to support flexible bitwidths for DNN operations
%
Stripes does not support or benefit from deep quantization of activations and it only leverages the quantization of weights. 
%
We compare our solution in terms of energy consumed and inference execution time against the 8-bit quantized network.

\vspace{-0.5cm}
\paragraph{Comparison with prior work.} 
%
We also compare against prior work~\cite{Ye2018AUF}, which proposes an iterative optimization procedure (dubbed ADMM) through which they find quantization bitwidths only for AlexNet and LeNet. 
%
Using Stripes~\cite{stripes} and TVM~\cite{TVM}, we show that \releq's solution provides higher performance and energy benefits compared to ADMM~\cite{Ye2018AUF}. 
%

\begin{table}
	\centering
	\caption{Hyper-Parameters of PPO used in ReLeQ.}
	
	\includegraphics[width=0.95\linewidth]{figs/hyperparam_table.pdf}
	\label{table:ppo_params}
	\vspace{-0.5cm}
\end{table}

\vspace{-0.5cm}
\paragraph{Implementation and hyper-parameters of the Proximal Policy Optimization (PPO).}
%
As discussed, \releq use PPO~\cite{ppo} as its RL engine, which we implemented in python where its policy and value networks use TensorFlow's Adam Optimizer with an initial learning rate of $10^{-4}$. 
%
The setting of the other hyper-parameters of PPO is listed in Table~\ref{table:ppo_params}.




==> body/methodology_new.tex <==
\section{RL for Deep Quantization of DNNs}
\label{sec:rl_quantization}
%\vspace{-1ex}

%\niparagraph{Need for heterogeneity.}
\subsection{Need for Heterogeneity}
%
Deep neural networks, by construction, and the underlying training algorithms cast different properties on different layers as they learn different levels of features representations. First, it is widely known that neural networks are heavily overparameterized~\cite{NIPS2019_8847}; thus, different layers exhibit different levels of redundancy. 
%
Second, for a given initialization and upon training, each layer exhibits a distribution of weights (typically bell-shaped) each of which has a different dynamic range leading to different degrees of robustness to quantization error, hence, different/heterogenous precision requirements. 
%
Third, our experiments (see Figure~\ref{fig:enum}), where the design space of deep quantization is enumerated for small and moderate size networks, empirically shows that indeed Pareto optimal frontier is mostly composed of heterogenous bitwidths assignment. 
%
Furthermore, recent works empirically studied the layer-wise functional structure of overparameterized deep models and provided evidence for the heterogeneous characteristic of  layers. 
%
Recent experimental work~\cite{DBLP:journals/corr/abs-1902-01996} also shows that layers can be categorized as either ``ambient'' or ``critical'' towards post-training re-initialization and re-randomization.
%
Another work~\cite{DBLP:conf/nips/FrommPP18} showed that a heterogeneously quantized versions of modern networks with the right mix of different bitwidths can match the accuracy of homogeneous versions with lower effective bitwidth on average.
%
All aforementioned points poses a requirement for methods to efficiently discover heterogenous bitwidths assignment for neural networks.
% 
However, exploiting this possibility is manually laborious~\cite{Micikevicius2017MixedPT, Mishra2017ApprenticeUK,DBLP:journals/corr/abs-1812-00090} as to preserve accuracy, the bitwidth varies across individual layers and different DNNs~\cite{Zhou2016DoReFaNetTL, Zhu2016TrainedTQ, Li2016TernaryWN, Mishra2017WRPNWR}.
%
Next subsection describes how to formulate this problem as a multi-objective optimization solved through Reinforcement Learning.


%\begin{comment}
\begin{figure}
 	\centering 	
 	\includegraphics[width=0.35\textwidth]{figs/sketch2.eps}
	%\caption{Optimum Automatic Quantization of a Neural Network}
	\caption{Sketch of the multi-objective optimization problem of layer-wise quantization of a neural network showing the underlying search space and the different design components.}
	\label{fig:intro}
%	\vspace{-0.5cm}
 \end{figure}
 %
%Figure \ref{fig:intro} shows a sketch of this search space and describes assignment of quantization level to each layer as a multi-objective optimization problem.
% --------------------------------------
\subsection{Multi-Objective Optimization} 
%
Figure \ref{fig:intro} shows a sketch of the multi-objective optimization problem of layer-wise quantization of a neural network showing the underlying search space and the different design components.
%
Given a particular network architecture, different patterns of layer-wise quantization bitwidths form a network specific design space (possible solutions).
%
Pareto frontier (\ballnumber{1}) defines the optimum patterns of layer-wise quantization bitwidths (Pareto optimal solutions). 
%
%Ideally (given enough time), a good search algorithm can find the best solution (i.e. on Pareto frontier).
% +++
However, not all Pareto optimal solutions are equally of interest as the accuracy objective has a priority over the quantization objective.
%
In the context of neural network quantization, preferred/desired region on the Pareto frontier for a given neural network is motivated by how recoverable the accuracy is for a given state of quantization (i.e., a particular pattern of layer-wise bitwidths) of the network.
% +++
Practically, the amount of recoverable accuracy loss (upon quantization) is determined by many factors: (1) the quantized training algorithm; (2) the amount of finetuning epochs; (3) the particular set of used hyperparameters; (4) the amenability of the network to recover accuracy, which is determined by the network architecture and how much overparameterization it exhibits.
%
As such, a constraint (\ballnumber{2}) is resulted below which even solutions on Pareto frontier are not interesting as they yield either unrecoverable or unaffordable accuracy loss depending on the application in hand.
%
%Therefore, in the context of neural networks quantization, the desirable region on Pareto frontier for a given neural network is motivated by how recoverable the accuracy is for a given state of quantization.
%
%Thus, the desirable region on Pareto frontier for a given neural network is motivated by how recoverable the accuracy is for a given state of quantization.
%
%In the context of neural networks quantization, preferred/desired region on the Pareto frontier for a given neural network is motivated by how recoverable the accuracy is for a given state of quantization (i.e., a particular pattern of layer-wise bitwidths) of the network.
%
%Theoretically, if it is possible to recover any loss in accuracy, then the lowest bitwidth option would be the optimum solution. Practically, the amount of recoverable accuracy loss is determined by many factors: first, the quantized training algorithm; second, the amount of training/finetuning epochs; third, particular set of used hyper-parameters; fourth, the amenability of the network to recover accuracy, which is determined by the network architecture and how much redundancy/overparameterization it exhibits.
%
%As such, considering all the above-mentioned factors, a constraint (labeled \ballnumber{3}) is resulted below which even solutions on the Pareto frontier are not interesting as they yield either unrecoverable or unaffordable accuracy loss depending on the application in hand.
%
We formulate this as a Reinforcement Learning (RL) problem where, by tuning a parametric reward function (\ballnumber{3}), the RL agent can be guided towards solutions around the desirable region (\ballnumber{4}) that strike a particular balance between the \bench{``State of Relative Accuracy''} (y-axis) and the \bench{``State of Quantization''} (x-axis).
%
%We formulate this as a Reinforcement Learning (RL) problem where the RL agent can be guided towards solutions in the desirable region (\ballnumber{4}) by tuning a parametric reward function (\ballnumber{3}) that strikes a particular balance between the \bench{``State of Relative Accuracy''} (y-axis) and the \bench{``State of Quantization''} (x-axis).
%\end{comment}
%
As such, \releq is an automated method for efficient exploration of large hyper-parameter space (heterogeneous bitwidths assignments) that is orthogonal to the underlying quantized training technique, quantization method, network architecture, and the particular hardware platform.
%
Changing one or more of these components could yield different search spaces, hence, different results.
% --------------------------------------
\if 0
%
For the sake of illustration, Figure \ref{fig:intro} shows a sketch of the multi-objective optimization problem of layer-wise quantization of a neural network showing the underlying search space and the different design components.
%
Given a particular network architecture, different patterns of layer-wise quantization bitwidths form a network specific design space (possible solutions).
%
Pareto frontier (labeled \ballnumber{1}) defines the optimum patterns of layer-wise quantization bitwidths (best solutions). 
%
%Ideally (given enough time), a good search algorithm can find the best solution (i.e. on Pareto frontier).
%
In the context of neural network quantization, preferred/desired region on the Pareto frontier for a given neural network is motivated by how recoverable the accuracy is for a given state of quantization (i.e., a particular pattern of layer-wise bitwidths) of the network.
%
Theoretically, if it is possible to recover any loss in accuracy, then the lowest bitwidth option would be the optimum solution. Practically, the amount of recoverable accuracy loss is determined by many factors: first, the quantized training algorithm; second, the amount of training/finetuning epochs; third, particular set of used hyper-parameters; fourth, the amenability of the network to recover accuracy, which is determined by the network architecture and how much redundancy/overparameterization it exhibits.
%
As such, considering all the above-mentioned factors, a constraint (labeled \ballnumber{3}) is resulted below which even solutions on the Pareto frontier are not interesting as they yield either unrecoverable or unaffordable accuracy loss depending on the application in hand.
%
This can be formulated as a Reinforcement Learning (RL) problem where the RL agent can be guided towards solutions in the desirable region (labeled \ballnumber{4}) by tuning a parametric reward function (labeled \ballnumber{2}) that strikes a particular balance between the \bench{``State of Relative Accuracy''} (y-axis) and the \bench{``State of Quantization''} (x-axis).
%\end{comment}
%
As such, \releq is an automated method for efficient exploration of large hyper-parameter space (heterogeneous bitwidths assignments) that is orthogonal to the underlying quantized training technique, quantization method, and network architecture.
%
Changing one or more of these components will yield different search spaces, hence, different results.
%
\fi 
%\vspace{-0.1cm}
\subsection{Method Overview} \releq trains a reinforcement learning agent that determines the level of deep quantization (below 8 bits) for each layer of the network.
%
\releq agent explores the search space of the quantization levels (bitwidths), layer by layer.
%
To account for the interplay between the layers with respect to quantization and accuracy, the state space designed for \releq comprises of both static information about the layers and dynamic information regarding the network state during the RL process (Section~\ref{sec:state}).
%
In order to consider the effects of previous layers' quantization levels, the agent steps sequentially through the layers and chooses a  bitwidth from a predefined set, e.g., $\{2, 3, 4, 5, 6, 7, 8\}$, one layer at a time (Section~\ref{sec:action}).
%
The agent, consequently, receives a reward signal that is proportional to its accuracy after quantization and its benefits in terms of computation and memory cost.
%
The underlying optimization problem is multi-objective (higher accuracy, lower compute, and reduced memory); however, preserving the accuracy is the primary concern.
%
To this end, we shape the reward asymmetrically to incentivize accuracy over the quantization benefits (Section~\ref{sec:reward}).
%
With this formulation of the RL problem, \releq employs the state-of-the-art Proximal Policy Optimization (PPO)~\cite{ppo} to train its policy and value networks.
%
This section details the components and the research path we have examined to design them.


\subsection{State Space Embedding to Consider Interplay between Layers}
\label{sec:state}
%\vspace{-1ex}

\if 0
\begin{table}
  \centering
  \caption{Layer and network parameters for state embedding.}
  \label{table:state_embed}
  \includegraphics[width=0.43\textwidth]{figs/state_embed.pdf}
%  \vspace{-0.5cm}
\end{table}
\fi 
% =================
\renewcommand{\arraystretch}{1.2}
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\begin{table}[htbp]
%\vspace{-0.5cm}
\centering
\small
\caption{Layer and network parameters for state embedding.}
%\vspace{-0.3cm}
\begin{center}
%\setlength\tabcolsep{1.5pt}
%\begin{tabular}{|P{0.7cm}|P{0.7cm}|M{0.8cm}|M{1.2cm}|c|c|c|}
\begin{tabularx}{\columnwidth}{YYY}
\toprule
%\multirow{2}{*}{PPO Clipping Parameter} & \multicolumn{3}{*}Average Normalized Reward (Performance) \\
& \bf Layer Specific & \bf Network Specific \\
\midrule
\multirow{4}{*}{\bf Static} & Layer index & \multirow{4}{*}{N/A} \\
\cline{2-2} 
& Layer Dimensions & \\
\cline{2-2} 
& \makecell {Weight Statistics \\ (standard deviation)} & \\
\midrule
\multirow{3}{*}{\bf Dynamic} &  \multirow{3}{*} {\makecell{Quantization Level \\ (Bitwidth)}} & State of Quantization \\
\cline{3-3} 
&& State of Accuracy \\
% & \bf LeNet on MNIST & \bf SimpleNet on CIFAR10 & \bf 8-Layers on SVHN \\
\bottomrule
%\textbf{Table}&\multicolumn{3}{|c|}{\textbf{Table Column Head}} \\
%\cline{2-4} 
%\textbf{Head} & \textbf{\textit{Table column subhead}}& \textbf{\textit{Subhead}}& \textbf{\textit{Subhead}} \\
%\hline
%copy& More table copy$^{\mathrm{a}}$& &  \\
%\hline
%\multicolumn{4}{l}{$^{\mathrm{a}}$Sample of a Table footnote.}
\end{tabularx}
%\vspace{-0.5cm}
\label{table:state_embed}
\end{center}
\end{table}
% =================

\niparagraph{Interplay between layers.} 
%
The final accuracy of a DNN is the result of interplay between its layers and reducing the bitwidth of one layer can impact how much another layer can be quantized.
%
Moreover, the sensitivity of accuracy varies across layers.
%
%Fully capturing such a complex interplay and sensitivity is both impractical and an overkill.
%
We design the state space and the actions to consider these sensitivities and interplay by including the knowledge about the bitwidth of previous layers, the index of the layer-under-quantization, layer size, and statistics (e.g., standard deviation) about the distribution of the weights.
%
However, this information is incomplete without knowing the accuracy of the network given a set of quantization levels and state of quantization for the entire network.
%
Table~\ref{table:state_embed} shows the parameters used to embed the state space of \releq agent, which are categorized across two different axes.
%
(1) \bench{``Layer-Specific''} parameters which are unique to the layer vs. \bench{``Network-Specific''} parameters that characterize the entire network as the agent steps forward during training process.
%
(2) \bench{``Static''} parameters that do not change during the training process vs. \bench{``Dynamic''} parameters that change during training depending on the actions taken by the agent while it explores the search space. 


\vspace{0.1cm}
\niparagraph{State of quantization and relative accuracy.}
%
The \bench{``Network-Specific''} parameters reflect some indication of the state of quantization and relative accuracy.
%
\bench{State of Quantization} is a metric to evaluate the benefit of quantization for the network and it is calculated using the compute cost and memory cost of each layer.
%
For a neural network with $L$ layers, we define compute cost of layer $l$ as the number of \textit{M}ultiply-\textit{Acc}umulate ($MAcc$) operations ($n^{MAcc}_l$), where ($l = 0, ..., L$).
%
Additionally, since \releq only quantizes weights, we define memory cost of layer $l$ as the number of weights ($n^w_l$) scaled by the ratio of \textit{Memory Access Energy} ($E_{MemoryAccess}$) to \textit{MAcc Computation Energy} ($E_{MAcc}$), which is estimated to be around $120\times$ \cite{TETRIS}. 
%
It is intuitive to consider that the sum of memory and compute costs linearly scale with the number of bits for each layer ($n^{bits}_l$). 
%
The $n^{bits}_{max}$ term is the maximum bitwidth among the predefined set of bitwidths that's available for the RL agent to pick from. 
%
Lastly, the \bench{State of Quantization} ($State_{Quantization}$) is the normalized sum over all layers ($L$) that accounts for the total memory and compute cost of the entire network.
%
%\begin{tiny}
%\vspace{-2ex}
%\[ State_{Quantization} = \frac{\sum_{l=0}^{L}\lbrack(n^w_l\times \frac{E_{MemoryAccess}}{E_{MAcc}}+n^{MAcc}_l)\times n^{bits}_l\rbrack}{\sum_{l=0}^{L}\lbrack n^w_l\times \frac{E_{MemoryAccess}}{E_{MAcc}}+n^{MAcc}_l\rbrack\times n^{bits}_{max}} \]
%\end{tiny}%
%
\begin{dmath}
 State_{Quantization} =  \frac{\sum_{l=0}^{L}\lbrack(n^w_l\times \frac{E_{MemoryAccess}}{E_{MAcc}}+n^{MAcc}_l)\times n^{bits}_l\rbrack}{\sum_{l=0}^{L}\lbrack n^w_l\times \frac{E_{MemoryAccess}}{E_{MAcc}}+n^{MAcc}_l\rbrack\times n^{bits}_{max}}
\end{dmath}
%
Besides the potential benefits, captured by $State_{Quantization}$, \releq considers the \bench{State of Relative Accuracy} to gauge the effects of quantization on the classification performance.
%
To that end, the \bench{State of Relative Accuracy} ($State_{Accuracy}$) is defined as the ratio of the current accuracy ($Acc_{Curr}$) with the current bitwidths for all layers during RL training, to accuracy of the network when it runs with full precision ($Acc_{FullP}$).
%
$State_{Accuracy}$ represents the degradation of accuracy as the result of quantization. 
%
%The closer this term is to $1.0$, the lower the accuracy loss and more desirable the quantization levels.
The closer this term is to $1.0$, the lower the accuracy loss and the more desirable/feasible the quantization.
%
%\begin{small}
%\vspace{-1ex}
%\[ State_{Accuracy} = \frac {Acc_{Curr}}{Acc_{FullP}} \]
%\end{small}
%\vspace{-2ex}
%
\begin{dmath}
State_{Accuracy} = \frac {Acc_{Curr}}{Acc_{FullP}} 
\end{dmath}
%
Given these embedding of the observations from the environment, the \releq agent can take actions, described next.

\subsection{Flexible Actions Space}
\label{sec:action}
%\vspace{-1ex}

\begin{figure}
    \centering
    \includegraphics[width=0.425\textwidth]{figs/action_space.png}
    \caption{(a) Flexible action space (used in \releq). (b)  Alternative action space with restricted movement.}		  
    \label{fig:action_space}
    %\vspace{0.2cm}
    \vspace{-0.2cm}
\end{figure}

%\paragraph{Action space for flexible exploration.} 
%
Intuitively, as calculations propagate through the layers, the effects of quantization will accumulate. 
%
As such, the \releq agent steps through each layer sequentially and chooses from the bitwidth of a layer from a discrete set of quantization levels which are provided as possible choices.
%
Figure~\ref{fig:action_space}(a) shows the representation of action space in which the set of bitwidths is $\{1, 2, 3, 4, 5, 6, 7, 8\}$. 
%
As depicted, the agent can flexibly choose to change the quantization level of a given layer from any bitwidth to any other bitwidth.
%
The set of possibilities can be changed as desired. 
%
Nonetheless, the action space depicted in Figure~\ref{fig:action_space}(a) is the possibilities considered for deep quantization in this work.
%
As illustrated in Figure~\ref{fig:action_space}(b), an alternative that we experimented with was to only allow the \releq agent to increment/decrement/keep the current bitwidth of the layer ($B^{(t)}$).
%
The experimentation showed that the convergence is much longer than the aforementioned flexible action space, which is used, as it encourages more exploration. 

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{figs/reward_shapes.pdf}
    \caption{Reward shaping with three different formulations as functions of the optimization objectives: state of relative accuracy and state of quantization. (a) Proposed formulation, (b) direct division, and (c) direct subtraction. The color palette shows the intensity of the reward.}
    \label{fig:reward_shapes}
%    \vspace{-0.5cm}
\end{figure}


\subsection{Asymmetric Reward Formulation for Accuracy}
\label{sec:reward}
%\vspace{-1ex}

While the state space embedding focused on interplay between the layers and the action space provided flexibility, reward formulation for \releq aims to preserve accuracy and minimize bitwidth of the layers simultaneously.
%
This requirement creates an asymmetry between the accuracy and bitwidth reduction, which is a core objective of \releq.
%
The following \bench{Reward Shaping} formulation provides the asymmetry and puts more emphasis on  maintaining the accuracy as illustrated with different color intensities in Figure~\ref{fig:reward_shapes}(a). 
%
This reward uses the same terms of \bench{State of Quantization} ($State_{Quantization}$) and \bench{State of Relative Accuracy} ($State_{Acc}$) from Section~\ref{sec:state}.
%
\input{listings/algorithm.tex}
%
One of the reasons that we chose this formulation is that it produces a smooth reward gradient as the agent approaches the optimum quantization combination.
%
In addition, the varying 2-dimensional gradient speeds up the agent's convergence time.
%
In the reward formulation, $a=0.2$ and $b=0.4$ can also be tuned and $th=0.4$ is threshold for relative accuracy below which the accuracy loss may not be recoverable and those quantization levels are completely unacceptable.
%
The use of threshold also accelerates learning as it prevents unnecessary or undesirable exploration in the search space by penalizing the agent when it explores undesired low-accuracy states.
%
While Figure~\ref{fig:reward_shapes}(a) shows the aforementioned formulation, Figures~\ref{fig:reward_shapes}(b) and (c) depict two other alternatives. 
%
Figure~\ref{fig:reward_shapes}(b) is based on $State_{Acc}/State_{Quantization}$ while Figure~\ref{fig:reward_shapes}(c) is based on  $State_{Acc} - State_{Quantization}$.
%  
Section~\ref{sec:rewardsens} provides detailed experimental results with these three reward formulations.
%
In summary, the formulation for Figure~\ref{fig:reward_shapes}(a) offers faster convergence. 
%
% The threshold also enables the agent to explore more relevant regions within the design space.
%
\begin{figure*}
    \centering
%    \includegraphics[width=0.9\textwidth]{figs/overview_new.pdf}
    \includegraphics[width=0.9\textwidth]{figs/overview_fig.pdf}
    \caption{Overview of \releq, which starts from a pre-trained network and delivers its corresponding deeply quantized network.}
    %, the layers of which use bitwidth below 8 bits.
    \label{fig:overview}
%    \vspace{-0.5cm}
\end{figure*}
%
\begin{figure}
  	  \centering\includegraphics[width=0.45\textwidth]{figs/releq_lenet_policy.pdf}
	  %\caption{Evolution of the ReLeQ agent bitwidth selection probabilities on MNIST dataset}
	  \caption{Action (Bitwidths selection) probability evolution over training episodes for LeNet.}
	  \label{fig:releq_lenet_policy}
%	  \vspace{-0.5cm}
 \end{figure}
%
\subsection{Policy and Value Networks}
%\vspace{-1ex}
%
While state, action and reward are three essential components of any RL problem, Policy and Value complete the puzzle and encode learning in terms of a RL context. 
%
While there are both policy-based and value-based learning techniques, \releq uses a state-of-the-art policy gradient based approach, Proximal Policy Optimization (PPO)~\cite{ppo}.
%
PPO is an actor-critic style algorithm so \releq agent consists of both Policy and Value networks.
%
%Because all the layers in a network are linked with each other and a decision at the beginning of the network impacts other layers, we use a LSTM based neural network architecture.

\subsection{Network Architecture of Policy and Value Networks}
%
Both Policy and Value are functions of state, so the state space defined in Section~\ref{sec:state} is encoded as a vector and fed as input to a Long short-term memory (LSTM) layer and this acts as the first hidden layer for both Policy and Value networks. 
%
Apart from the LSTM, policy network has two fully connected hidden layers of 128 neurons each and the number of neurons in the final output layer is equal to the number of available bitwidths the agent can choose from. Whereas the Value network has two fully connected hidden layers of 128 and 64 neurons each. 
%
Based on our evaluations, LSTM enables the \releq agent to converge almost $\times{1.33}$ faster in comparison to a network with only fully connected layers.
%

While this section focused on describing the components of \releq in isolation, the next section puts them together and shows how \releq automatically quantizes a pre-trained DNN.



==> body/outlook.tex <==
\section{Accelerated Finetuning}
%
 %\niparagraph{Loss function of neural networks.}
 \paragraph{Loss function of neural networks.}
 %
 Neural networks' loss functions are known to be highly non-convex and generally very poorly understood. It has been empirically verified that loss surfaces for large neural networks have many local minima that are essentially equivalent in terms of test error \cite{DBLP:journals/corr/ChoromanskaHMAL14}, \cite{DBLP:journals/corr/abs-1712-09913}. 
%
Moreover, converging to one of the many good local minima proves to be more useful as compared to struggling to find the global minimum of the accuracy loss on the training set (which often leads to overfitting). This opens up and encourages a possibility of adding extra custom objectives to optimize for (during the training process), in addition to the original one (accuracy loss). The added custom objective could be with the purpose of increasing generalization performance or imposing some preference on the weights values. 
%
Regularization is one of the major techniques that makes use of such facts as discussed in the following subsection.
 
 %


%\niparagraph{Quantization friendly regularization.}
\paragraph{Quantization friendly regularization.}
%
Neural networks often suffer from redundancy of parameterization and consequently they commonly tend to overfit.
%
Regularization is one of the commonly used techniques to enhance generalization performance of neural networks.
%
Regularization effectively constrains weight parameters by adding a term (regularizer) to the objective function that captures the desired constraint in a soft way. This is achieved by imposing some sort of preference on weights updates during the optimization process. As a result, regularization seamlessly leads to unconditionally constrained optimization problem instead of explicitly constrained which, in most cases is much more difficult to solve.
%
The most commonly used regularization technique is known as \textit{weight decay}, which aims to reduce the network complexity by limiting the growth of the weights. It is realized by adding a term to the objective function that penalizes large weight values \cite{Krogh:1991:SWD:2986916.2987033}:
\[ E(w) = E_o(w) + \frac{1}{2} \lambda \sum\limits_{i} {w_i}^2 \]

where $E_o$ is the original loss measure, and $\lambda$ is a parameter governing how strongly large weights are penalized. $w$ is a vector containing all free parameters of the network.
%

%\begin{figure}[t]
%	\centering
%	\subfloat[t][]{\includegraphics[width=0.35\textwidth]{figs/quant_friendly_a.pdf}
%		\label{fig:quant_a}}
%	\subfloat[t][]{\includegraphics[width=0.29\textwidth]{figs/quant_friendly_b.pdf}
%		\label{fig:quant_b}}
%	\subfloat[t][]{\includegraphics[width=0.25\textwidth]{figs/quant_friendly_c.pdf}
%		\label{fig:quant_c}}
%	\caption{Quantization friendly regularization.}
%	\label{fig:sin2_reg}
%\end{figure}



\begin{figure}[t]
\centering
\begin{subfigure}{0.35\textwidth}
  \centering\includegraphics[width=\textwidth]{figs/quant_friendly_a.pdf}
		\caption{some caption}
		\label{fig:quant_a}
\end{subfigure}

\begin{subfigure}{0.29\textwidth}
  \centering\includegraphics[width=\textwidth]{figs/quant_friendly_b.pdf}
	\caption{some caption}
		\label{fig:quant_b}
\end{subfigure}

\begin{subfigure}{0.25\textwidth}
  \centering\includegraphics[width=\textwidth]{figs/quant_friendly_c.pdf}
  \caption{some caption}
	\label{fig:quant_c}
\end{subfigure}
\caption{Quantization friendly regularization.}
\label{fig:sin2_reg}
\end{figure}


{\setlength{\parindent}{0cm}Here, we propose a new type of regularization that is friendly to quantization. The proposed regularization is realized by adding a periodic function (regularizer) to the original objective function, Figure \ref{fig:quant_a}. The periodic regularizer has a periodic pattern of minima that correspond to the desired quantization levels. Such correspondence is achieved by matching the period to the quantization step based on a particular number of bits for a given layer.}
\[ E(w) = E_o(w) + \frac{1}{2} \lambda_{q} \sum\limits_{i} {\sin^{2}\left({\frac {\pi w_i} {2^{-qbits}}}\right)} \]
where $E_o$ is the original loss measure, and $\lambda_q$ is a parameter governing how strongly weight quantization errors are penalized. $w$ is a vector containing all free parameters of the network.
%

For the sake of simplicity and clarity, Figures \ref{fig:quant_b} and \ref{fig:quant_c} depict a geometrical sketch for a hypothetical loss surface (original objective function to be minimized) and an extra regularization term in 2-D weight space. 
For weight decay regularization, in Figure \ref{fig:quant_b}, the faded circular contours show that as we get closer to the origin, the regularization loss is minimized. Optimum solution is achieved by striking a balance between the original loss term and the regularization loss term.
%
In a similar way, Figure \ref{fig:quant_c} shows a representation of the proposed regularization. A periodic pattern of minima pockets is seen surrounding the original optimum point. The objective of the optimization problem is to find the best solution that is the closest to one of those minima pockets where weight values are nearly matching the desired quantization levels, hence the name quantization-friendly.
%

%\niparagraph{Evaluation.}
\paragraph{Evaluation.}
%
To demonstrate the effectiveness of the proposed regularization, Figure \ref{fig:sin2_eval_1} shows a comparison of the validation accuracy for CIFAR-10 using conventional finetuning approach versus finetuning with the proposed approach. It can be noticed that, under same limited amount of retraining steps, medium number of bits seem to benefit the most. Observed performance improvements could differ across different networks and different durations of retraining.
%
It should be noted that, using the proposed regularization approach, the weight updates occur in full precision as opposed to clipping the weights to the quantized values, yet the weights eventually converge to desired quantization levels.
 

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{figs/val_accuracy.pdf}
    \caption{Comparison of validation accuracy of CIFAR-10 after retraining for 10k steps at different quantization bitwidths for weights (assuming same bitwidth for all layers).}		  
    \label{fig:sin2_eval_1}
    \vspace{0.2cm}
\end{figure}




==> body/related.tex <==
\section{Related Work}
\vspace{-1ex}
%
ReLeQ is the initial step in utilizing reinforcement learning to automatically find the level of quantization for the layers DNNs such that their classification accuracy is preserved.
%
As such, it relates to the techniques that given a level of quantization, train a neural network or develop binarized DNNs.
%
Furthermore, the line of research that utilizes RL for hyper-parameter discovery and tuning inspires \releq.
%
Nonetheless, \releq, uniquely and exclusively, offers an RL-based approach to determine the levels of quantization.


\niparagraph{Training algorithms for quantized neural networks.}
%
There have been several techniques~\cite{Zhou2016DoReFaNetTL, Zhu2016TrainedTQ, Mishra2017WRPNWR} that train a neural network in a quantized domain after the bitwidth of the layers is determined manually.
%
DoReFa-Net \cite{Zhou2016DoReFaNetTL} trains quantized convolutional neural networks with parameter gradients which are stochastically quantized to low bitwidth numbers before they are propagated to the convolution layers. \cite{Mishra2017WRPNWR} introduces a scheme to train networks from scratch using reduced-precision activations by decreasing the precision of both activations and weights and increasing the number of filter maps in a layer. 
%
\cite{Zhu2016TrainedTQ} performs the training phase of the network in full precision, but for inference uses ternary weight assignments. For this assignment, the weights are quantized using two scaling factors which are learned during training phase.
%
PACT \cite{Choi2018PACTPC}  introduces a quantization scheme for activations, where the variable $\alpha$ is the clipping level and is determined through a gradient descent based method.

ReLeQ is an orthogonal technique with a different objective: automatically finding the level of quantization that preserves accuracy and can potentially use any of these training algorithms.  

\niparagraph{Binarized neural networks.}
%
Extensive work, \cite{Hubara2017QNN, Rastegari2016XNORNetIC, Li2016TernaryWN} focuses on binarized neural networks, which impose accuracy loss but reduce the bitwidth to lowest possible level.
%
In BinaryNet \cite{NIPS2016BNN}, an extreme case, a method is proposed for training binarized neural networks which reduce memory size, accesses and computation intensity at the cost of accuracy.
%
XNOR-Net \cite{Rastegari2016XNORNetIC} leverages binary operations (such as XNOR) to approximate convolution in binarized neural networks. 
%
%BinaryNet and XNOR-Net alleviate most of the multiplications needed in the forward and backward passes of the network and thereby achieve high performance in comparison to full-precision networks. 
%
Another work \cite{Li2016TernaryWN} introduces ternary-weight networks, in which the weights are quantized to {-1, 0, +1} values by minimizing the Euclidian distance between full-precision weights and their ternary assigned values.
%
\releq aims to utilize the levels between binary and 8 bits to avoid loss of accuracy while offering automation.

\niparagraph{Reinforcement learning for hyper-parameter tuning.}
%
Few works leverage RL in the context of hyper-parameter search.
%
Two of these inspiring efforts~\cite{Zoph2016NeuralAS, Baker2016DesigningNN} use RL to determine the architecture of the neural network and its kernels.
%
%The former uses policy a gradient method whereas the latter employs Q-learning. 
%
Another research~\cite{He2018AMCAF} employs an RL policy gradient method to automatically find the compression ratio for different layers of a network. 

%Compared to previous works, our initial version \cite{ReLeQ} is the first study that combines the two approaches and proposes an automated reinforcement learning based approach for bitwidth selection in the context of neural network quantization.

\niparagraph{Techniques for selecting quantization levels.}
%
Recent work ADMM~\cite{Ye2018AUF} runs a binary search to minimize the total square quantization error in order to decide the quantization levels for the layers. Then, they use an iterative optimization technique for fine-tuning.
%
NVIDIA also released an automatic mixed precision (AMP)~\cite{nvidia_auto} which employs mixed precision during training by automatically selecting between two floating point (FP) representations (FP16 or FP32).
%
%Although it is an interesting effort, it is different than our study in a sense that it only considers two representations.

There is a concurrent work HAQ~\cite{HAQ} which also uses RL in the context of quantization.
%
The following highlights some of the differences.
%
\releq uses a unique reward formulation and shaping that enables simultaneously optimizing for two objectives (accuracy and reduced computation with lower-bitwidth) within a unified RL process.
%
In contrast, HAQ utilizes accuracy in the reward formulation and then adjusts the RL solution through an approach that sequentially decreases the layer bitwidths to stay within a predefined resource budget.
%
This approach also makes HAQ focused more towards a specific hardware platform whereas we are after a strategy than can generalize.
%
%Additionally, \releq uses Proximal Policy Optimization~\cite{ppo} while the other work utilizes Deep Deterministic Policy Gradient~\cite{DDPG}.
%
Additionally, we also provide a systemic study of different design decisions, and have significant performance gain across diverse well known benchmarks.
%
%The initial version of our work~\cite{ReLeQ}, predates HAQ, and it is the first to use RL for quantization.
The initial version of our work~\cite{DBLP:journals/corr/abs-1811-01704}, predates HAQ, and it is the first to use RL for quantization.
%
%The initial version of our work~\cite{ReLeQ}, predates HAQ, and it is the first to use RL for quantization\footnote{We have disclosed our arXiv paper to the program committee chairs while anonymizing it in the references.}.


